Low-Level Augmented Bayesian Optimization for Finding the Best Cloud VM

With the advent of big data applications, which tends to have longer execution time, choosing the right cloud VM to run these applications has significant performance as well as economic implications. For example, in our large-scale empirical study of 107 different workloads on three popular big data systems, we found that a wrong choice can lead to a 20 times slowdown or an increase in cost by 10 times. Bayesian optimization is a technique for optimizing expensive (black-box) functions. Previous attempts have only used instance-level information (such as # of cores, memory size) which is not sufficient to represent the search space. In this work, we discover that this may lead to the fragility problem---either incurs high search cost or finds only the sub-optimal solution. The central insight of this paper is to use low-level performance information to augment the process of Bayesian Optimization. Our novel low-level augmented Bayesian Optimization is rarely worse than current practices and often performs much better (in 46 of 107 cases). Further, it significantly reduces the search cost in nearly half of our case studies. Based on this work, we conclude that it is often insufficient to use general-purpose off-the-shelf methods for configuring cloud instances without augmenting those methods with essential systems knowledge such as CPU utilization, working memory size and I/O wait time.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=IEEEtran
NAME=paper

TEX = abstract.tex bo.tex approach.tex conclusion.tex evaluation.tex introduction.tex background.tex paper.tex relatedwork.tex

PDF = $(PACKAGE).pdf

all:  $(NAME).pdf


paper.pdf: paper.tex $(PACKAGE).cls $(PACKAGE).bst $(TEX)
	pdflatex $<
	- bibtex -min-crossrefs=999 $(NAME) 
	pdflatex $<
	- bibtex -min-crossrefs=999 $(NAME)
	pdflatex $<

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls $(PACKAGE).bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

